New Approximation Bounds for Small-Set Vertex Expansion

The vertex expansion of the graph is a fundamental graph parameter. Given a graph $G=(V,E)$ and a parameter $\delta \in (0,1/2]$, its $\delta$-Small-Set Vertex Expansion (SSVE) is defined as \[ \min_{S : |S| = \delta |V|} \frac{|{\partial^V(S)}|}{ \min \{ |S|, |S^c| \} } \] where $\partial^V(S)$ is the vertex boundary of a set $S$. The SSVE~problem, in addition to being of independent interest as a natural graph partitioning problem, is also of interest due to its connections to the Strong Unique Games problem. We give a randomized algorithm running in time $n^{{\sf poly}(1/\delta)}$, which outputs a set $S$ of size $\Theta(\delta n)$, having vertex expansion at most \[ \max\left(O(\sqrt{\phi^* \log d \log (1/\delta)}) , \tilde{O}(d\log^2(1/\delta)) \cdot \phi^* \right), \] where $d$ is the largest vertex degree of the graph, and $\phi^*$ is the optimal $\delta$-SSVE. The previous best-known guarantees for this were the bi-criteria bounds of $\tilde{O}(1/\delta)\sqrt{\phi^* \log d}$ and $\tilde{O}(1/\delta)\phi^* \sqrt{\log n}$ due to Louis-Makarychev [TOC'16]. Our algorithm uses the basic SDP relaxation of the problem augmented with ${\rm poly}(1/\delta)$ rounds of the Lasserre/SoS hierarchy. Our rounding algorithm is a combination of the rounding algorithms of Raghavendra-Tan [SODA'12] and Austrin-Benabbas-Georgiou [SODA'13]. A key component of our analysis is novel Gaussian rounding lemma for hyperedges which might be of independent interest.

==> header.tex <==
In this part, we prove the following SSEH based hardness for \ssve.

\ssvehard*

The reduction for the above theorem starts with the following (conjectured) hard instances of {\sc SmallSetEdgeExpansion}.

\begin{definition}[$(\tilde{\epsilon},\tilde{\delta},\tilde{C})$-\sse]
	Given parameters $\tilde{\epsilon},\tilde{\delta} \in (0,1)$ and $\tilde{C} \in [1,\infty)$, an $(\tilde{\epsilon},\tilde{\delta},\tilde{C})$-\sse~instance is characterized by a graph $G = (V,E)$ and the goal here is to distinguish between the following two cases:
	\begin{itemize}
		\item {\bf YES Case}: There exists a set $S \subset V$ such that ${\sf Vol}(S) = \tilde{\delta}$ we have $\phi_G(S) \leq \tilde{\epsilon}$.
		\item {\bf NO Case}: For every set $S \subset V$ such that ${\sf Vol}(S) \in \left[\frac{\tilde{\delta}}{\tilde{C}},\tilde{C}\tilde{\delta}\right]$, we have $\phi_G(S) \geq 1  - \tilde{\epsilon}$.
	\end{itemize}	
\end{definition}

Our reduction uses the hard instances from the following conjecture.

\begin{conjecture}[Small Set Expansion Hypothesis~\cite{RST12}]				\label{conj:sse}					
	For any $\tilde{\epsilon} \in (0,1)$ and $M \in [1,\infty)$, there exists $\tilde{\delta} = \tilde{\delta}(\tilde{\epsilon},M)$ such that $(\tilde{\epsilon},\tilde{\delta},M)$-\sseh~is \NP-Hard.
\end{conjecture}

Theorem \ref{thm:ssve-hard} follows directly by combining Conjecture \ref{conj:sse} and the following theorem which gives a factor preserving reduction from \smallsetexpansion~to \ssve.

\begin{theorem}					\label{thm:ssve-redn}
	The following holds any choice of $\epsilon,\delta \in (0,1)$ and $d \geq 2$ satisfying $\epsilon \in \left[1/d^{100},1/d\right]$ and $d \geq 4\log(1/\epsilon\delta)$. Let $\tilde{\epsilon} = (\epsilon \delta)^{4d^2/\epsilon^3}$ and $\tilde{C} = (\epsilon \delta)^{-2d^2/\epsilon^3}$. Then there exists a randomized polynomial time reduction from $(\tilde{\e},\tilde{\delta},\tilde{C})$-\smallsetexpansion~instances $G = (V,E)$ to \ssve~instances $G'' = (V'',E'')$ such that the following properties hold.
	\begin{itemize}
		\item If $G$ is a YES instance, then $\phi^{V}_{\delta}(G'') \leq \epsilon$.
		\item If $G$ is a NO instance, the $\phi^{V}_\delta(G'') \geq \sqrt{\epsilon\log d\log(1/\delta)}$.
	\end{itemize}
	Moreover the degree of $G''$ is bounded by ${\rm poly}(d)$.
\end{theorem}

\begin{remark}
	In the above theorem, we can actually take $\epsilon \geq 1/d^L$ for any large constant $L$.
\end{remark}

{\bf Outline}. The proof of the above theorem proceeds in stages, we briefly outline the structure of the proof below for the reader's convenience.

\begin{itemize}
	\item In Section \ref{sec:aexp-redn}, we describe the reduction from \smallsetexpansion~to $(d,\delta)$-\avexp (i.e., an analytic variant of symmetric vertex expansion). Sections \ref{sec:aexp-comp} and \ref{sec:aexp-sound} establish the completeness and soundness directions of the reduction.
	\item Section \ref{sec:unif} gives a factor preserving reduction from \avexp~instances to \avexp~instances with uniform weights.
	\item Section \ref{sec:sub-samp} gives a factor preserving reduction from \avexp~instances with uniform weights to {\sc SymmetricSSVE}.
\end{itemize}

